Semantic Soundness for Language Interoperability

Programs are rarely implemented in a single language, and thus questions of type soundness should address not only the semantics of a single language, but how it interacts with others. Even between type-safe languages, disparate features frustrate interoperability, as invariants from one language can easily be violated in the other. In their seminal 2007 paper, Matthews and Findler proposed a multi-language construction that augments the interoperating languages with a pair of boundaries that allow code from one language to be embedded in the other. While the technique has been widely applied, their syntactic source-level interoperability doesn't reflect practical implementations, where behavior of interaction is defined after compilation to a common target, and any safety must be ensured by target invariants or inserted target-level "glue code." In this paper, we present a framework for the design and verification of sound language interoperability that follows an interoperation-after-compilation strategy. Language designers specify what data can be converted between types of the languages via a relation $\tau_A \sim \tau_B$ and specify target glue code implementing conversions. Then, by giving a semantic model of source types as sets of target terms, we can establish soundness of conversions: i.e., whenever $\tau_A \sim \tau_B$, the corresponding pair of conversions convert target terms that behave as $\tau_A$ to target terms that behave as $\tau_B$, and vice versa. We can then prove semantic type soundness for the entire system. We illustrate our framework via a series of case studies that demonstrate how our semantic interoperation-after-compilation approach allows us both to account for complex differences in language semantics and make efficiency trade-offs based on particularities of compilers or targets.

==> case-affdyn.tex <==
\section{Affine \& Unrestricted}\label{sec:affdyn}

In our third case study, we consider an affine language, $\langatlc$,
interacting with an unrestricted one, $\langref$. In this case, unlike the
previous one, the substructural features from $\langatlc$ can be enforced
dynamically, which means we can allow more flexible but sound mixing than would
be possible if the types were linear. In particular, we adopt the classic
technique, described in \cite{tov10}, where affine resources are protected
behind thunks with stateful flags that indicate failure on a second force.


\paragraph{Languages} We present the syntax of $\langref$ and $\langatlc$ and
the static semantics of $\langatlc$ in Fig.~\ref{fig:affdyn-syntax}; we elide
the static semantics of $\langref$, which are standard. As in the previous case
studies, we will support open terms across language boundaries, and thus need to
carry environments for both languages. However, while with $\langsysf$ and
$\langlt$, the only sound option was to disallow linear resources from crossing
boundaries, in this case study, we can protect affine resources. That means that
our affine \mbox{environments $\alang{\Affenv}$ need to be split, even within
$\langref$, to respect the affine invariant.}

Rather than splitting environments from the other language, we instead adopt a
generic method for threading these types of contexts, where each judgment has an
input and output context from the foreign language. i.e., a typing rule for
$\langatlc$ will have the shape $\rlang{\context};\alang{\Gamma};\alang{\Affenv}
\vdash \alang{e} : \alang{\tau} \produces \rlang{\context'}$, where
$\rlang{\context}$ stands for all of the static typing environments needed by
$\langref$. So, $\acolor{\context} = \alang{\Gamma};\alang{\Omega}$ and
$\rlang{\context} = \rcolor{\Delta};\rcolor{\Gamma}$. Since each judgment has
both input and output,
and we thread this through subterms, this allows not only unrestricted
judgments (which do not change the output) but substructural ones (which do
change the output), in a reasonably lightweight way.

\begin{figure}[t!]
  \begin{small}
    \[
      \begin{array}{llcl}
        \langatlc &
        \text{Type~}\alang{\tau} & ::= & \alang{unit \vo bool \vo int \vo \tau \multimap \tau \vo ~!\tau \vo
          \tau \& \tau \vo \tau \otimes \tau} \\
        & \text{Expression~}\alang{e} & ::= & \alang{() \vo true \vo false \vo n \vo  x \vo a \vo \lambda a : \tau . e \vo e
          ~ e}  \vo \alang{\lconvert}\rlang{e}\alang{\rconvert_{\tau}} \alang{\vo ~!e }\\
        & & & \alang{\vo let~ !x = e ~in~ e' \vo \langle e, e' \rangle \vo e.1 \vo e.2 \vo (e,e) \vo let~ (a,a') = e ~in~ e'} \\
        & \text{Value~}\alang{v} & ::= & \alang{() \vo \lambda a : \tau . e \vo ~!e \vo \langle e, e'
          \rangle \vo (v,v')}\\
        \langref &
        \text{Type~} \rlang{\tau} & ::= & \rlang{unit} \vo  \rlang{int} \vo \rlang{\tau \times \tau}
        \vo \rlang{\tau + \tau} \vo \rlang{\tau
          \rightarrow \tau} \vo \rlang{\forall\alpha.\tau \vo \alpha}
        \vo \rlang{ref~\tau}\\

        & \text{Expression~} \rlang{e} & ::= & \rlang{()} \vo \rlang{\mathbb{Z}} \vo \rlang{x} \vo \rlang{(e,e)} \vo
        \rlang{fst~e} \vo \rlang{snd~e}  \vo
        \rlang{inl~e} \vo \rlang{inr~e} \vo
        \rlang{match~e~x\{e\}~y\{e\}} \\
        & & & \vo \rlang{\lambda x : \tau.e} \vo \rlang{e~e} \vo
        \rcolor{\Lambda\alpha.\mathtt{e}} \vo \rlang{e{[}\tau{]}} \vo
        \rlang{ref~e} \vo \rlang{!e} \vo \rlang{e := e} \vo \rlang{\convert{\tau}{\alang{e}}}
      \end{array}
    \]
      \begin{mathpar}
  \inferrule{\alang{a} : \alang{\tau} \in \alang{\Affenv} }{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{a} :
    \alang{\tau} \produces \rlang{\context}}
\and
\inferrule{\alang{x} : \alang{\tau} \in \alang{\Gamma}}{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash
  \alang{x} : \alang{\tau}\produces \rlang{\context}}
\and
\inferrule{ }{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{n} : \alang{int}\produces \rlang{\context}}
\and
\inferrule{\alang{\Gamma};\alang{\Affenv};\rcolor{\Delta};\rcolor{\Gamma} \vdash \rlang{e} : \rlang{\tau} \produces \alang{\Gamma};\alang{\Affenv'}\\ \_ : \alang{\tau} \conv
  \rlang{\tau}}{\rcolor{\Delta};\rcolor{\Gamma};\alang{\Gamma};\alang{\Affenv} \vdash \alang{\lconvert}\rlang{e}\alang{\rconvert_{\tau}} :
  \alang{\tau}\produces \rcolor{\Delta};\rcolor{\Gamma}}
\quad
\inferrule{\alang{\Affenv} = \alang{\Affenv\alang{_1} \uplus \Affenv\alang{_2}} \\ \rlang{\context_1};\alang{\Gamma};\alang{\Affenv}\alang{_1} \vdash \alang{e_1} : \alang{\tau_1 \multimap
    \tau_2}\produces \rlang{\context_2} \\ \rlang{\context_2};\alang{\Gamma};\alang{\Affenv}\alang{_2} \vdash \alang{e_2} :
  \alang{\tau_1}\produces \rlang{\context_3}}{\rlang{\context_1};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e_1 ~ e_2}  : \alang{\tau_2}\produces \rlang{\context_3}}
\and
\inferrule{\rlang{\context};\alang{\Gamma};\cdot \vdash \alang{e} : \alang{\tau}\produces \rlang{\context'}}{\rlang{\context};\alang{\Gamma};\cdot
  \vdash \alang{!e} : \alang{!\tau}\produces \rlang{\context'}}
\and
\inferrule{\alang{\Affenv} = \alang{\Affenv\alang{_1} \uplus
    \alang{\Affenv}\alang{_2}}
  \\\rlang{\context_1};\alang{\Gamma};\alang{\Affenv}\alang{_1} \vdash
  \alang{e} : \alang{!\tau}\produces \rlang{\context_2}
  \\
  \rlang{\context_2};\alang{\Gamma[x := \tau]};\alang{\Affenv}\alang{_2} \vdash \alang{e'} :
  \alang{\tau'}\produces \rlang{\context_3}}{\rlang{\context_1};\alang{\Gamma};\alang{\Affenv} \vdash
  \alang{let~ !x = e ~in~ e'}\produces \rlang{\context_3}}
\and
\inferrule{\rlang{\context_1};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e_1} : \alang{\tau_1} \produces \rlang{\context_2}\\
  \rlang{\context_2};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e_2} :
  \alang{\tau_2}\produces \rlang{\context_3}}{\rlang{\context_1};\alang{\Gamma};\alang{\Affenv} \vdash
  \alang{\langle e_1, e_2 \rangle} : \alang{\tau_1 \& \tau_2}\produces \rlang{\context_3}}
\and
\inferrule{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e} : \alang{\tau_1 \&
    \tau_2}\produces \rlang{\context'}}{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e.1} : \alang{\tau_1}\produces \rlang{\context'}}
\and
\inferrule{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e} : \alang{\tau_1 \&
    \tau_2}\produces \rlang{\context'}}{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{e.2} : \alang{\tau_2}\produces \rlang{\context'}}
\and
\inferrule{\rlang{\context};\alang{\Gamma};\alang{\Affenv[a := \tau_1]} \vdash \alang{e} :
  \alang{\tau_2}\produces \rlang{\context'}}{\rlang{\context};\alang{\Gamma};\alang{\Affenv} \vdash \alang{\lambda a : \tau_1. e} :
  \alang{\tau_1 \multimap \tau_2}\produces \rlang{\context'}}
\and
\inferrule{\alang{\Affenv} = \alang{\Affenv\alang{_1} \uplus \alang{\Affenv}\alang{_2}} \\\rlang{\context_1};\alang{\Gamma};\alang{\Affenv}\alang{_1} \vdash \alang{e_1} : \alang{\tau_1}\produces \rlang{\context_2} \\
  \rlang{\context_2};\alang{\Gamma};\alang{\Affenv}\alang{_2} \vdash \alang{e_2} :
  \alang{\tau_2}\produces \rlang{\context_3}}{\rlang{\context_1};\alang{\Gamma};\alang{\Affenv} \vdash
  \alang{(e_1, e_2)} : \alang{\tau_1 \otimes \tau_2}\produces \rlang{\context_3}}
\and
\inferrule{\alang{\Affenv} = \alang{\Affenv\alang{_1} \uplus \alang{\Affenv}\alang{_2}}
  \\ \rlang{\context_1};\alang{\Gamma};\alang{\Affenv}\alang{_1} \vdash \alang{e} : \alang{\tau_1 \otimes \tau_2} \produces \rlang{\context_2}\\
  \rlang{\context_2};\alang{\Gamma};\alang{\Affenv_2[a := \tau_1, a' := \tau_1]}
  \vdash \alang{e'} : \alang{\tau'}\produces \rlang{\context_3}}{\rlang{\context_1};\alang{\Gamma};\alang{\Affenv} \vdash
  \alang{let~ (a,a') = e ~in~ e'} : \alang{\tau'}\produces \rlang{\context_3}}
\end{mathpar}
\vspace{-0.25cm}
    \caption{Syntax for $\langref$; syntax \& selected statics for $\langatlc$.}
    \label{fig:affdyn-syntax}
  \end{small}
\end{figure}


Returning to Fig.~\ref{fig:affdyn-syntax}, we can see that $\langatlc$
maintains an affine environment, introduced by lambda and tensor-destructuring
let, that it splits across subterms, but it does not require that all bindings be
used, as we can see in the terminal rules for variables (affine $\alang{a}$ and
unrestricted $\alang{x}$), unit, booleans, etc.



Our target language is the same untyped lambda calculus, $\langtarget$
(Fig.~\ref{fig:polylin-target}), from our previous case study. Our compilers,
presented in Fig.~\ref{fig:affdyn-compilers}, are primarily interesting in the
cases that address affine bindings; otherwise, they do standard type erasure for
polymorphic types, etc. We use a compiler macro, $\thnk(\cdot)$,
which expands to a nullary function 
closing over a freshly-allocated reference---called a \emph{flag}---initialized to $\tlang{1}$.
When called, this function fails if the flag is set to $\tlang{0}$.
Otherwise, it sets the flag to $\tlang{0}$ and returns the macro's argument.
Throughout the paper, we will use the constants $\aunused$ and $\aused$ for $1$
and $0$.
We use $\thnk(\cdot)$ when introducing affine bindings, 
and then we compile uses of affine variable to expressions that force the thunk.
Unrestricted $\langatlc$ variables $\alang{x}$
and variables from $\langref$ are unaffected by this strategy.

\begin{figure}
  \begin{small}
    \[
    \begin{array}[t]{lcl}
      \rlang{()} & \rightsquigarrow & \tlang{()}\\
      \rlang{\mathbb{Z}} & \rightsquigarrow & \tlang{\mathbb{Z}}\\
      & & \\
      & & \\
      \rlang{x} & \rightsquigarrow & \tlang{x}\\
      & & \\
      \rlang{\lambda x : \tau.e} & \rightsquigarrow & \tlang{\lambda x.\{\rlang{e^\tlang{+}}\}}\\
      \rlang{e_1~e_2} & \rightsquigarrow & \tlang{\rlang{e_1^\tlang{+}}~\rlang{e_2^\tlang{+}}}\\
      \rlang{(e_1,e_2)} & \rightsquigarrow & \tlang{(\rlang{e_1^\tlang{+}},\rlang{e_2^\tlang{+}})}\\
      \rlang{fst~e} & \rightsquigarrow & \tlang{fst~\rlang{e^\tlang{+}}}\\
      \rlang{snd~e}  & \rightsquigarrow & \tlang{snd~\rlang{e^\tlang{+}}}\\
      \rlang{inl~e} & \rightsquigarrow & \tlang{inl~\rlang{e^\tlang{+}}}\\
      \rlang{inr~e} & \rightsquigarrow & \tlang{inr~\rlang{e^\tlang{+}}}\\
      \rlang{match~e}& \rightsquigarrow & \tlang{match~\rlang{e^\tlang{+}}}\\
        \enspace\rlang{x\{e_1\}~y\{e_2\}} & & \enspace \tlang{x\{\rlang{e_1^\tlang{+}}\}~y\{\rlang{e_2^\tlang{+}}\}} \\
      \rcolor{\Lambda\alpha.\rlang{e}} & \rightsquigarrow & \tlang{\lambda \_.\{\rlang{e^\tlang{+}}\}}\\
      \rlang{e{[}\tau{]}} & \rightsquigarrow &\tlang{\rlang{e^\tlang{+}}~()}\\
      \rlang{ref~e} & \rightsquigarrow & \tlang{ref~\rlang{e^\tlang{+}}}\\
      \rlang{!e} & \rightsquigarrow & \tlang{!\rlang{e^\tlang{+}}}\\
      \rlang{e_1 := e_2} & \rightsquigarrow & \tlang{\rlang{e_1^\tlang{+}} := \rlang{e_2^\tlang{+}}}\\
      \rlang{\convert{\tau}{\alang{e}}} & \rightsquigarrow & C_{\alang{\tau}{\mapsto}\rlang{\tau}}(\alang{e^\tlang{+}})\\
    \end{array}
    \begin{array}[t]{lcl}
      \alang{()} & \rightsquigarrow & \tlang{()} \\
      \alang{n} & \rightsquigarrow & \tlang{n} \\
      \alang{true} & \rightsquigarrow & \tlang{0}\\
      \alang{false} & \rightsquigarrow & \tlang{1}\\
      \alang{x} & \rightsquigarrow & \tlang{x}\\
      \alang{a} & \rightsquigarrow & \tlang{a~()}\\
      \alang{\lambda a : \tau . e} & \rightsquigarrow & \tlang{\lambda a. \{\alang{e^\tlang{+}}\}}\\
      \alang{e_1 ~ e_2}  & \rightsquigarrow & \tlang{\alang{e_1^\tlang{+}}~(let~x = \alang{e_2^\tlang{+}}~in~\thnk(x))}\\
      \alang{(e_1,e_2)} & \rightsquigarrow & \tlang{(\alang{e_1^\tlang{+}},\alang{e_2^\tlang{+}})}\\
      \alang{e.1} & \rightsquigarrow & \tlang{(fst~\alang{e^\tlang{+}})\, ()}\\
      \alang{e.2} & \rightsquigarrow & \tlang{(snd~\alang{e^\tlang{+}})\, ()}\\
      \alang{\langle e_1, e_2 \rangle} & \rightsquigarrow & \tlang{(\lambda \_.\{\alang{e_1^\tlang{+}}\},\lambda \_.\{\alang{e_2^\tlang{+}}\})}\\
      & & \\
      \alang{let~ (a_1,a_2) = e_1} & \rightsquigarrow & \tlang{let~x_{\text{fresh}}
                                                          =
                                                          \alang{e_1^\tlang{+}},~
                                                          x_{\text{fresh}}' = fst~x_{\text{fresh}},} \\
                                                          \enspace \alang{in~e_2} & & \enspace \tlang{x_{\text{fresh}}'' = snd~x_{\text{fresh}},~}
                                                          \tlang{a_1
                                                          = \thnk(x_{\text{fresh}}'),} \\
                                                          & & \enspace \tlang{a_2
                                                          = \thnk(x_{\text{fresh}}'')~in~\alang{e_2^\tlang{+}}}\\
      \alang{!e} & \rightsquigarrow & \tlang{\alang{e^\tlang{+}}}\\
      \alang{let~ !x = e_1} & \rightsquigarrow & \tlang{let~x = \alang{e_1^\tlang{+}}~in~\alang{e_2^\tlang{+}}}\\
        \enspace \alang{in~e_2} & & \\
      & & \\
      \alang{\lconvert}\rlang{e}\alang{\rconvert_{\tau}} & \rightsquigarrow & C_{\rlang{\tau}{\mapsto}\alang{\tau}}(\rlang{e^\tlang{+}})
  \end{array}
  \]
  \[
    \thnk(\tlang{e}) \triangleq \tlang{let~r_{fresh} = ref~\aunused~in~}\lambda \_.\{
    \tlang{if~!r_{fresh}~\{\convfail\}~\{r_{fresh}:=\aused;e\}\}}\text{~where~}\aused=0\text{~and~}\aunused=1
  \]\vspace{-0.25cm}
    \caption{Compilers for $\langref$ and $\langatlc$.}
    \label{fig:affdyn-compilers}
  \end{small}
\end{figure}

\paragraph{Convertibility} We define convertibility relations and conversions
for $\langatlc$ and $\langref$ in Fig.~\ref{fig:affdyn-conv}. In it we define
base type conversions between $\alang{unit}$ and $\rlang{unit}$, $\alang{bool}$
and $\rlang{int}$, tensors and pairs, and between $\rlang{\rightarrow}$ and
$\alang{\multimap}$. The last is most interesting and challenging. Our compiler
is designed to support affine code being mixed directly with unrestricted code.
Intuitively, an affine function should be able to behave as an unrestricted one,
but the other direction is harder to accomplish, and higher-order functions mean
both must be addressed at once. In order to account for this, we convert
$\alang{\tau_1 \multimap \tau_2}$ not to $\rlang{\tau_1 \rightarrow \tau_2}$
(not even for some convertible argument/return types), but rather to
$\rlang{(unit \rightarrow \tau_1) \rightarrow \tau_2}$. That is, to a $\langref$
function that expects its argument to be a thunk containing a $\rlang{\tau_1}$
rather than a $\rlang{\tau_1}$ directly. Provided that the thunk fails if
invoked more than once, we can ensure, dynamically, that a $\langref$ function
with that type behaves as an $\langatlc$ function of a related type. These
invariants are ensured by appropriate wrapping and use of the compiler macro
$\thnk(\cdot)$.



\begin{figure}
  \begin{small}
\[
      \begin{array}{l@{~}c@{~~~}l}
        Atom_n &\triangleq& \{ (\W,\tlang{e_1},\tlang{e_2}) \vo \W \in World_n \} \quad
        AtomVal_n \triangleq \{ (\W,\tlang{v_1},\tlang{v_2}) \in Atom_n \} \quad
        \mathit{AtomVal} \triangleq \bigcup_n \mathit{AtomVal}_n\\
        \mathit{World}_n &\triangleq& \{(k,\heapty,\astore) \vo k < n \land \heapty \subset
        \mathit{HeapTy}_k\land \dom{\heapty} \# \dom{\astore}\}\\
        \mathit{HeapTy}_n &\triangleq& \{(\loc_1,\loc_2) \mapsto \mathit{Typ}_{n}, \ldots \}\\
        Typ_n &\triangleq& \{ R \in 2^{AtomVal_n} \vo \forall (\W,\tlang{v_1},\tlang{v_2}) \in R.~\forall\W'.~ \W
        \worldext \W' \implies (\W',\tlang{v_1},\tlang{v_2}) \in R  \}\\
        Typ &\triangleq& \{ R\in 2^{AtomVal} \vo \forall k. \floor{k}{R}\in Typ_k \}\\
        \astore &\triangleq& \{(\loc_1,\loc_2) \mapsto \{\aused,\aunused\}, \ldots \}
        \text{~where~}\aused=0~\text{and}~\aunused=1\\
        \W \worldext \W' &\triangleq& \begin{array}[t]{l}
          \W'.k \le \W.k \land~ \forall (\loc_1,\loc_2) \in \dom{\W.\heapty}.
        \floor{\W'.k}{\W.\heapty(\loc_1,\loc_2)} = \W'.\heapty(\loc_1,\loc_2) \\
        \land~ \forall (\loc_1,\loc_2) \in \dom{\W.\astore}.(\loc_1,\loc_2) \in \dom{\W'.\astore} \land
        (\W.\astore(\loc_1,\loc_2) = \aused \implies \W'.\astore(\loc_1,\loc_2)
        = \aused)\\
        \end{array}\\
        \heap_1,\heap_2 : \W &\triangleq&   (\forall (\loc_1,\loc_2) \mapsto R \in \W.\heapty.~(\later \W,\heap_1(\loc_1),\heap_2(\loc_2)) \in R) \land\ (\forall
        (\loc_1,\loc_2) \mapsto b \in \W.\astore.\heap_1(\loc_1) = \heap_2(\loc_2) = b)\\
      \end{array}
    \]    \[
\begin{array}{lcl}
  \Vrel{\rlang{\mathtt{unit}}}{\rho} &=& \{(\W,\tlang{()},\tlang{()}) \}\\
  \Vrel{\rlang{\mathtt{int}}}{\rho} &=& \{(\W,\tlang{n},\tlang{n}) \vo \tlang{n} \in
  \mathbb{Z}  \}\\
  \Vrel{\rlang{\tau_1 \times \tau_2}}{\rho} &=& \{(\W,
  (\tlang{v_{1a}},\tlang{v_{2a}}), (\tlang{v_{1b}},\tlang{v_{2b}})) \vo
  (\W, \tlang{v_{1a}}, \tlang{v_{1b}}) \in \Vrel{\rlang{\tau_1}}{\rho} \land
  (\W,\tlang{v_{2a}}, \tlang{v_{2b}}) \in \Vrel{\rlang{\tau_2}}{\rho}
  \}\\
  \Vrel{\rlang{\tau_1 + \tau_2}}{\rho} &=& \{(\W, \tlang{inl~v_1}, \tlang{inl~v_2})
  \vo (\W,\tlang{v_1},\tlang{v_2}) \in \Vrel{\rlang{\tau_1}}{\rho} \} ~\cup~
  \{(\W,\tlang{inr~v_1}, \tlang{inr~v_2} )
  \vo  (\W,\tlang{v_1},\tlang{v_2})
  \in \Vrel{\rlang{\tau_2}}{\rho} \}\\
  \Vrel{\rlang{\tau_1 \rightarrow \tau_2}}{\rho} &=&
  \{(\W,\tlang{\lambda x.\{e_1\}}, \tlang{\lambda x.\{e_2\}}) \vo
  \forall \tlang{v_1}~\tlang{v_2}~ \W'. \W \worldextstrict \W'~ \land~
  (\W',\tlang{v_1},\tlang{v_2}) \in \Vrel{\rlang{\tau_1}}{\rho} \\ & &
  \implies (\W', [x {\mapsto} \tlang{v_1}]\tlang{e_1}, [x {\mapsto} \tlang{v_2}]\tlang{e_2}) \in \Erel{\rlang{\tau_2}}{\rho}
  \}\\
  \Vrel{\rlang{\mathtt{ref}~\tau}}{\rho} &=& \{(\W,\tlang{\loc_1},\tlang{\loc_2})
  \vo
  \W.\heapty(\loc_1,\loc_2) = \floor{\W.k}{\Vrel{\rlang{\tau}}{\rho}} \}\\
  \Vrel{\rlang{\forall\alpha.\tau}}{\rho} &=&
  \{(\W,\tlang{\lambda\_.e_1}, \tlang{\lambda\_.e_2}) \vo
  \forall R \in Typ,~\W'. \W \worldextstrict \W'\implies (\W',\tlang{e_1},\tlang{e_2}) \in \Erel{\rlang{\tau}}{\rho[\alpha \mapsto
    R]}\}\\
  \Vrel{\rlang{\alpha}}{\rho} &=& \rho(\alpha)\\
    \Vrel{\alang{unit}}{\cdot} &=& \{(\W,\tlang{()},\tlang{()})\}\\
    \Vrel{\alang{bool}}{\rho} &=& \{(\W,0,0)\} \cup \{(\W,\tlang{n_1},\tlang{n_2})
    \vo n_1 \ne 0 \land n_2 \ne 0  \}\\
  \Vrel{\alang{int}}{\cdot} &=& \{(\W,\tlang{n},\tlang{n}) \vo  \tlang{n} \in \mathbb{Z}\}\\
  \Vrel{\alang{\tau_1 \multimap \tau_2}}{\cdot} &=&
  \{(\W,\tlang{\lambda~a. e_1},\tlang{\lambda~a. e_2}) \vo \forall \tlang{v_1}~\tlang{v_2}~ \W'~\ell_1~\ell_2. \\ & &
  ~~\W \worldextstrict \W' \land
  (\W',\tlang{v_1},\tlang{v_2}) \in \Vrel{\alang{\tau_1}}{\cdot} \land (\ell_1, \ell_2)\notin\dom{\W'.\heapty}\cup\dom{\W'.\astore} \\ & &
  \implies ((\W'.k, \W'.\heapty, \W'.\astore \uplus (\ell_1,\ell_2) \mapsto \aunused),\\ & & \quad [\tlang{a} {\mapsto}
  \grd(\tlang{v_1},\ell_1)]\tlang{e_1}, [\tlang{a} {\mapsto}
  \grd(\tlang{v_2},\ell_2)]\tlang{e_2}) \in \Erel{\alang{\tau_2}}{\cdot}
    \}\\
    \Vrel{\alang{!\tau}}{\cdot} &=& \{(\W, \tlang{v_1}, \tlang{v_2}) \vo (\W, \tlang{v_1}, \tlang{v_2}) \in \Vrel{\alang{\tau}}{\cdot}\}\\
    \Vrel{\alang{\tau_1 \otimes \tau_2}}{\cdot} &=& \{(\W,
    \tlang{(v_{1a},v_{2a})}, \tlang{(v_{1b},v_{2b})}) \vo
    (\W,\tlang{v_{1a}}, \tlang{v_{1b}}) \in \Vrel{\alang{\tau_1}}{\cdot} \land
    (\W,\tlang{v_{2a}}, \tlang{v_{2b}}) \in \Vrel{\alang{\tau_2}}{\cdot}
    \}\\
    \Vrel{\alang{\tau_1 \& \tau_2}}{\cdot} &=& \{(\W, (\tlang{\lambda
      \_.\{e_{1a}\}},\tlang{\lambda \_.\{e_{2a}\}}), (\tlang{\lambda \_.\{e_{1b}\}},\tlang{\lambda \_.\{e_{2b}\}}))
    \\ & & \quad \vo
    (\W,\tlang{e_{1a}},\tlang{e_{1b}}) \in \Erel{\alang{\tau_1}}{\cdot} \land
    (\W,\tlang{e_{2a}}, \tlang{e_{2b}}) \in \Erel{\alang{\tau_2}}{\cdot}
    \}
\end{array}
\]
\[
  \grd(e,\ell) \triangleq \lambda \_.\{
  \tlang{if~!\ell~\{\convfail\}~\{\ell:=\aused;e\}\}}
\]
    \[
      \begin{array}{l}
        \Erel{\tau}{\rho} = \{(\W,\tlang{e_1},\tlang{e_2}) \vo
        \fv(\tlang{e_1}) = \fv(\tlang{e_2}) = \emptyset ~\land\\
        \qquad \forall \heap_1,\heap_2 {:} \W,~ \tlang{e_1'},~ \heap_1',~ j <
        \W.k.~
        \tconf{\heap_1}{\tlang{e_1}} \steps{j} \tconf{\heap_1'}{\tlang{e_1'}} \nrightarrow \\
        \qquad
        \implies
        \tlang{\tlang{e_1'}} = \tlang{\convfail}
        \lor
        (\exists \tlang{v_2} \heap_2' \W'.
        \tconf{\heap_2}{\tlang{e_2}} \steps{*} \tconf{\heap_2'}{\tlang{v_2}} \land
        \W \worldext \W' \land \heap_1', \heap_2' : \W'
        \land  (\W', \tlang{e_1'},\tlang{v_2}) \in \Vrel{\tau}{\rho})\}
      \end{array}
    \]\vspace{-0.25cm}
    \caption{Logical Relation for $\langref$ and $\langatlc$.}
    \label{fig:affdyn-lr}
  \end{small}
\end{figure}

\paragraph{Semantic Model} To reason about this system, we present our step
indexed binary logical relation in Fig.~\ref{fig:affdyn-lr}. Although there is
some overlap with the previous case studies and prior work, the treatment of
affine resources is novel. In our worlds $W$s, we keep the step index, a standard heap
typing $\heapty$, which maintains a simple bijection between locations of the
two programs (which doesn't support sophisticated reasoning about equivalence in
the presence of ``local state''~\cite{ahmed09} but suffices for soundness), but
also an affine flag store, $\astore$, which maintains a bijection on flags
(locations) that track whether affine variables have been used. This is a subset
of the heap, disjoint from $\heapty$, and restricted by the model to only
contain either $0$ or $1$, which for convenience we write using the constants
$\aused$ and $\aunused$. Our world extension relation, $\W \worldext \W'$, shows
that flags cannot be removed from $\astore$, and once a flag is marked as
$\aused$, it cannot be marked $\aunused$. With this setup, our expression
relation $\Erel{\tau}\rho$ is quite ordinary, as the described structure is
entirely about characterizing the heaps that programs will run in, not about how
they will run. Note that $\Erel{\tau}\rho$ allows for the possibility of
$\tlang{e_1}$ raising a conversion error ($\tlang{\convfail}$) at runtime.

Finally, while most of the cases in our value relation are standard,
the affine arrow $\alang{\multimap}$ is novel. A pair of functions
$\tlang{\lambda a.e_1}$ and $\tlang{\lambda a.e_2}$ are related if, given a pair of arguments
$\tlang{v_1}$ and $\tlang{v_2}$ related at a future world $\W'$, we get related
results in $\W'$ extended with a new entry in the flag store $\W'.\astore$ for some
fresh locations $\loc_1,\loc_2$. Importantly, what we substitute into the body
is \emph{not} $\tlang{v_1}$ and $\tlang{v_2}$, but rather wrapped forms,
$\grd(\tlang{v_1},\loc_1)$ and $\grd(\tlang{v_2},\loc_2)$, each of which closes
over the fresh location in the flag store and thus ensures that the argument is not
used more than once. This makes sense, since in the target, we expect affine 
variables to be thunks, and will force them upon use.




\begin{figure}
  \begin{small}
    \begin{mathpar}
      \inferrule{
      }{C_{\rlang{unit}{\mapsto}\alang{unit}},C_{\alang{unit}{\mapsto}\rlang{unit}}
        : \rlang{unit} \conv \alang{unit}}

      \inferrule{
      }{C_{\rlang{int}{\mapsto}\alang{bool}},C_{\alang{bool}{\mapsto}\rlang{int}}
        : \rlang{int} \conv \alang{bool}}

      \inferrule{
        C_{\alang{\tau_1}{\mapsto}\rlang{\tau_1}},C_{\rlang{\tau_1}{\mapsto}\alang{\tau_1}}
        : \alang{\tau_1} \conv \rlang{\tau_1} \\ C_{\alang{\tau_2}{\mapsto}\rlang{\tau_2}},C_{\rlang{\tau_2}{\mapsto}\alang{\tau_2}}
        :\alang{\tau_2} \conv
        \rlang{\tau_2}}{C_{\alang{\tau_1\otimes\tau_2}{\mapsto}\rlang{\tau_1\times\tau_2}},C_{\rlang{\tau_1\times
            \tau_2}{\mapsto}\alang{\tau_1\otimes\tau_2}}
        :\alang{\tau_1 \otimes \tau_2} \conv
        \rlang{\tau_1 \times \tau_2}}


      \inferrule{        C_{\alang{\tau_1}{\mapsto}\rlang{\tau_1}},C_{\rlang{\tau_1}{\mapsto}\alang{\tau_1}}
        :\alang{\tau_1} \conv \rlang{\tau_1} \\ C_{\rlang{\tau_2}{\mapsto}\alang{\tau_2}},C_{\alang{\tau_2}{\mapsto}\rlang{\tau_2}}
        :\alang{\tau_2} \conv \rlang{\tau_2}}{
        C_{\alang{\tau_1\multimap\tau_2}{\mapsto}\rlang{(unit\rightarrow\tau_1)\rightarrow\tau_2}},C_{\rlang{(unit
            \rightarrow\tau_1)\rightarrow\tau_2}{\mapsto}\alang{\tau_1\multimap\tau_2}}
        :\alang{\tau_1 \multimap \tau_2} \conv \rlang{
          (unit \rightarrow \tau_1) \rightarrow \tau_2}}
    \end{mathpar}

    \[
    C_{\rlang{unit}{\mapsto}\alang{unit}}(\tlang{e}) \triangleq C_{\rlang{int}{\mapsto}\alang{bool}}(\tlang{e}) \triangleq
    C_{\alang{unit}{\mapsto}\rlang{unit}}(\tlang{e}) \triangleq
    \tlang{e} \quad
    C_{\alang{bool}{\mapsto}\rlang{int}}(\tlang{e}) \triangleq \tlang{if~e~0~1}
\]
\[\arraycolsep=2pt
  \begin{array}{lcl}
    \tlang{C}_{\alang{\tau_1 \otimes \tau_2}{\mapsto}\rlang{\tau_1 \times
        \tau_2}}\tlang{(e)} & \triangleq &
                                   \tlang{let~x=e~in~(}\tlang{C}_{\alang{\tau_1}{\mapsto}\rlang{\tau_1}}(\tlang{fst~x}),\tlang{C}_{\alang{\tau_2}{\mapsto}\rlang{\tau_2}}(\tlang{snd~x})\tlang{)}\\

    \tlang{C}_{\rlang{\tau_1 \times \tau_2}{\mapsto}\alang{\tau_1 \otimes
    \tau_2}}\tlang{(e)} &\triangleq&
                             \tlang{let~x=e~in~}\tlang{(}\tlang{C}_{\rlang{\tau_1}{\mapsto}\alang{\tau_1}}(\tlang{fst~x}),\tlang{C}_{\rlang{\tau_2}{\mapsto}\alang{\tau_2}}(\tlang{snd~x})\tlang{)}\\

     \tlang{C}_{\alang{\tau_1 \multimap \tau_2}{\mapsto}\rlang{(unit \rightarrow \tau_1) \rightarrow
         \tau_2}}\tlang{(e)} &\triangleq& \tlang{let~x=e~in~\lambda
       x_{thnk}.let~x_{conv} = \tlang{C}_{\rlang{\tau_1}{\mapsto}\alang{\tau_1}}(x_{thnk}~())}
     \\ & & \qquad \qquad \qquad \tlang{in~ let~x_{acc}=\thnk(x_{conv})
      ~in~\tlang{C}_{\alang{\tau_2}{\mapsto}\rlang{\tau_2}}(x~x_{acc})}\\

    \tlang{C}_{\rlang{(unit \rightarrow \tau_1) \rightarrow \tau_2}{\mapsto}\alang{\tau_1 \multimap
          \tau_2}}\tlang{(e)}
                                                     &\triangleq& \tlang{let~x=e~in~
          \lambda x_{thnk}. let~x_{acc}=\thnk(C_{\alang{\tau_1}\mapsto\rlang{\tau_1}}(x_{thnk}~()))~in~C_{\rlang{\tau_2}{\mapsto}\alang{\tau_2}}(\tlang{x~x_{acc}})}\\
    \end{array}
  \]\vspace{-0.25cm}
    \caption{Convertibility for $\langref$ and $\langatlc$.}
    \label{fig:affdyn-conv}
  \end{small}
\end{figure}

With the logical relation in hand, we can prove the following:

\begin{theorem}[Convertibility Soundness]\label{theorem:convertibilitysoundness}~\\
  \indent If $\rlang{\tau} \conv \alang{\tau}$ then
  $\begin{array}[t]{l}\forall~(\W, \tlang{e_1}, \tlang{e_2}) \in
  \Erel{\rlang{\tau}}{\cdot} \implies
  (\W,C_{\rlang{\tau}{\mapsto}\alang{\tau}}(\tlang{e_1}),C_{\rlang{\tau}{\mapsto}\alang{\tau}}(\tlang{e_2})) \in
  \Erel{\alang{\tau}}{\cdot}\\
  \forall~(\W, \tlang{e_1}, \tlang{e_2}) \in
  \Erel{\alang{\tau}}{\cdot} \implies
  (\W,C_{\alang{\tau}{\mapsto}\rlang{\tau}}(\tlang{e_1}), C_{\alang{\tau}{\mapsto}\rlang{\tau}}(\tlang{e_2})) \in \Erel{\rlang{\tau}}{\cdot}\end{array}$
\end{theorem}

\begin{theorem}[Fundamental Property]\label{theorem:affdyn-fund-prop}~

  If~ $\alang{\Gamma};\alang{\Affenv};\rcolor{\Delta}; \rcolor{\Gamma} \vdash \rlang{e : \tau} \produces \alang{\Gamma'}; \alang{\Affenv'}$ then
  $\alang{\Gamma};\alang{\Affenv};\rcolor{\Delta}; \rcolor{\Gamma} \vdash \rlang{e \aprx e : \tau} \produces \alang{\Gamma'}; \alang{\Affenv'}$ and if
  $~\rcolor{\Delta}; \rcolor{\Gamma}; \alang{\Gamma}; \alang{\Affenv} \vdash \alang{e : \tau} \produces \rcolor{\Delta'}; \rcolor{\Gamma'}$ then
  $\rcolor{\Delta}; \rcolor{\Gamma}; \alang{\Gamma}; \alang{\Affenv} \vdash \alang{e \aprx e : \tau}\produces \rcolor{\Delta'}; \rcolor{\Gamma'}$.
\end{theorem}

\begin{theorem}[Type Safety for
  $\langref$]\label{theorem:affdyn-langref-typesafe}~

  For any $\langref$ term $\rlang{e}$ where $\cdot; \cdot; \cdot; \cdot\vdash \rlang{e : \tau}\produces \cdot; \cdot$ and for any heap $\heap$, if $\tconf{\heap}{\rlang{e}^+} \steps{*} \tconf{\heap'}{\tlang{e'}}$, then either $\tlang{e'}=\convfail$, $\tlang{e'}$ is a value, or there exist $\heap'', \tlang{e''}$ such that $\tconf{\heap'}{\tlang{e'}}\step \tconf{\heap''}{\tlang{e''}}$.
\end{theorem}

\begin{theorem}[Type Safety for
  $\langatlc$]\label{theorem:affdyn-langatlc-typesafe}~

  For any $\langatlc$ term $\alang{e}$ where $\cdot; \cdot; \cdot; \cdot\vdash
  \alang{e : \tau}\produces \cdot; \cdot$ and for any heap $\heap$, if
  $\tconf{\heap}{\alang{e}^+} \steps{*} \tconf{\heap'}{\tlang{e'}}$, then we
  know from the logical relation that either $\tlang{e'}=\convfail$,
  $\tlang{e'}$ is a value, or there exist $\heap'', \tlang{e''}$ such that
  $\tconf{\heap'}{\tlang{e'}}\step \tconf{\heap''}{\tlang{e''}}$.
\end{theorem}



\paragraph{Examples.} Using our conversions, we investigate several small
examples, presented (with their compilations) in
Figure~\ref{fig:affdyn-examples}. Program $P1$ converts a $\langref$ function
that projects the first element of a pair of integers to $\langatlc$ and applies
it to $\alang{(true,false)}$, producing $\alang{true}$ successfully. By
contrast, $P1^\dagger$ tries to use the pair twice (sites of errors are \hl{highlighted}),
which once converted to $\langatlc$, is a violation of the type invariant, and
thus this produces a runtime error, which we can see in the compiled code will
occur at the second invocation of $\tlang{x~()}$, which contains the contents of
a $\thnk(\cdot)$.

Program $P2$ defines an affine function (and immediately applies it) that binds
a variable $\alang{a}$ in $\langatlc$, then uses it (inside a closure) in
$\langref$, returning a pair made up of that variable and a value from
$\langref$. This works fine, evaluating to $\alang{(true,true)}$. Program
$P2^\dagger$ attempts to do an analogous thing, but uses the variable twice,
which is a violation of the affine type and thus results in a runtime failure.
We can see that in the invocations of $\tlang{a~()}$, which contain $\thnk(0)$.


\begin{figure}
\begin{small}
  \[\arraycolsep=1pt\begin{array}{lcl}
    P1 &=&
    \alang{\lconvert}\rlang{(\lambda x:(unit \rightarrow int \times int). fst~(x~()))}\alang{\rconvert_{bool\otimes bool \multimap bool}~(true,false)}\\
  P1^\dagger &=& \alang{\lconvert}\rlang{(\lambda x:(unit
    \rightarrow int \times int). (fst~(x~()),snd~(\hl{x~()})))}\alang{\rconvert_{bool\otimes bool \multimap bool \otimes bool}~(true,false)}\\
  P2 &=& \alang{(\lambda a:bool.\lconvert}\rlang{(\lambda y:int.(\convert{int}{\alang{a}},y))~0}\alang{\rconvert_{bool\otimes bool})~true}\\
  P2^\dagger &=& \alang{(\lambda a:bool.\lconvert}\rlang{(\lambda y:int.(\convert{int}{\alang{a}},\convert{int}{\alang{\hl{a}}}))~0}\alang{\rconvert_{bool\otimes bool})~true}\\[0.5em]
      \text{compile}^*(P1) &=& \tlang{(\lambda
        x^1_{thnk}.} \tlang{(\lambda
        x.\{fst~(x~())\})~\thnk(let~x^2=(x^1_{thnk}~())~in~(if~(fst~x^2)~0~1,if~(snd~x^2)~0~1))}\\
      & & \hspace{1.1cm} \tlang{(\thnk((0,1)))}\\
      \text{compile}^*(P1^\dagger) &=&\tlang{(\lambda
        x^1_{thnk}.(let~x^3~=(\lambda
        x.\{(fst~(x~()),snd(\hl{x~()})\})}\\
      & & \hspace{2.3cm} \tlang{(\thnk(let~x^2=(x^1_{thnk}~())~in~(if~(fst~x^2)~0~1,if~(snd~x^2)~0~1)))} \\
      & & \hspace{1.1cm} \tlang{in~(fst~x^3,snd~x^3))}~\tlang{(\thnk((0,1)))} \\
      \text{compile}^*(P2) &=& \tlang{(\lambda a.(let~x^2=((\lambda y.(if~(a~())~0~1,y))~0)~in~(fst~x^2,snd~x^2)))~(let ~x^1=0~in~\thnk(x^1))} \\
      \text{compile}^*(P2^\dagger) &=& \tlang{(\lambda a.(let~x^2=((\lambda y.(if~(a~())~0~1,if~(\hl{a~()})~0~1))~0)~in~(fst~x^2,snd~x^2)))~(let ~x^1=0~in~\thnk(x^1))}
    \end{array}
  \]
  \text{Note: compile$^*(\cdot)$ performs basic simplifications after compiling.}
\vspace{-0.25cm}
\caption{Examples of interoperability for $\langref$ and $\langatlc$, with
  compilations.}
\label{fig:affdyn-examples}
\end{small}
\end{figure}

